Bucks for Buckets (B4B): Active Defenses Against Stealing Encoders

Machine Learning as a Service (MLaaS) APIs provide ready-to-use and high-utility encoders that generate vector representations for given inputs. Since these encoders are very costly to train, they become lucrative targets for model stealing attacks during which an adversary leverages query access to the API to replicate the encoder locally at a fraction of the original training costs. We propose Bucks for Buckets (B4B), the first active defense that prevents stealing while the attack is happening without degrading representation quality for legitimate API users. Our defense relies on the observation that the representations returned to adversaries who try to steal the encoder's functionality cover a significantly larger fraction of the embedding space than representations of legitimate users who utilize the encoder to solve a particular downstream task.vB4B leverages this to adaptively adjust the utility of the returned representations according to a user's coverage of the embedding space. To prevent adaptive adversaries from eluding our defense by simply creating multiple user accounts (sybils), B4B also individually transforms each user's representations. This prevents the adversary from directly aggregating representations over multiple accounts to create their stolen encoder copy. Our active defense opens a new path towards securely sharing and democratizing encoders over public APIs.

==> bib-backup.tex <==
@inproceedings{SSLextraction,
title={On the Difficulty of Defending Self-Supervised Learning against Model Extraction},
author={Dziedzic, Adam and Dhawan, Nikita and Kaleem, Muhammad Ahmad and Guan, Jonas and Papernot, Nicolas},
booktitle={International Conference on Machine Learning},
year={2022},
}

==> contents/checklist.tex <==
% \newpage
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% % The checklist follows the references.  Please
% % read the checklist guidelines carefully for information on how to answer these
% % questions.  For each question, change the default \answerTODO{} to \answerYes{},
% % \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% % justification to your answer}, either by referencing the appropriate section of
% % your paper or providing a brief inline description.  For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% % Please do not modify the questions and only use the provided macros for your
% % answers.  Note that the Checklist section does not count towards the page
% % limit.  In your paper, please delete this instructions block and only keep the
% % Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


% %The checklist must appear in the submitted PDF, immediately after references, but does not count towards the page limit.

% \begin{enumerate}

% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{See Appendix Section~\ref{sec:limitations}.}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{See Appendix Section~\ref{sec:negative-impact}.}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerYes{}
% \end{enumerate}

% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{Provided with the supplementary materials.}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{See Appendix~\ref{sec:additional-experiments}.}
% 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerYes{}
% 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{See Appendix~\ref{sec:additional-experiments}.}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{See Section \ref{sec:related-work}}
%   \item Did you mention the license of the assets?
%     \answerNo{All licences MIT.}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerYes{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerNo{Used datasets are either synthetic or popular standard datasets.}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNo{Used datasets are either synthetic or popular standard datasets.}
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}

% \end{enumerate}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> contents/intro_without_framework.tex <==
\section{Introduction}



%\adam{The text for this content should be moved from this google doc: \url{https://docs.google.com/document/d/15ExbuJ-raRVIF5MIUOMJ7t_oFPWzt3gRbsgMBlc8O1s/edit?usp=sharing}.}
In model stealing attacks, adversaries extract a machine learning model exposed via a public API by repeatedly querying it and updating their own model based on obtained responses. Model stealing is considered one of the main threats to the security of machine learning models~\citep{MicrosoftSurvey}.
%[]\tf{@Adam, please cite the Microsoty survey here}. \tf{maybe make clear that stealing and extraction means the same thing}
Since the introduction of the the first extraction attack against classifiers~\citep{tramer2016usenix}, a lot of work on improving stealing~\citep{kariyappa2021maze,orekondy2019knockoff,tramer2016usenix}, extending it to different model types~\cite{carlini2021extracting,shen2022model}, and proposing adequate defenses~\citep{powDefense,jia2021entangled,juuti2019prada,digital_wm} has been put forward.
With the recent shift in learning paradigms from supervised to self supervised learning (SSL), especially the need of new defenses becomes increasingly pressing.
From an academic viewpoint, the urge arises because it was shown that SSL models (\textit{encoders}) are even more vulnerable to model stealing~\citep{SSLextraction,StolenEncoder,ContSteal} than their supervised counterparts.
This is because whereas supervised models' output is low dimensional, \eg per-class probabilities or pure labels, SSL encoders output high-dimensional representation vectors that encode a larger amount information and thereby facilitate stealing.
In addition, from a practical industry's viewpoint, defenses are required since many popular API providers, such as Cohere, OpenAI, or Clarify~\citep{Clarifai,Cohere,OpenAI} already expose their high-value SSL encoders via APIs to a broad range of users.



% Model stealing attacks and defenses have become the new area of great interest from both research and industry viewpoints. 
% Since the dawn of the first work on model extraction~\citep{tramer2016usenix}, there has been an increasing effort to assess the threat of model stealing~\citep{jagielski2020fidelity} and a new spectrum of defenses~\citep{powDefense,juuti2019prada}. The new emerging paradigm of SSL encoders shifted the focus to the emerging APIs that return representations for given inputs instead of low-dimensional outputs~\citep{Clarifai,Cohere,OpenAI}. Recent work showed that SSL encoders are even more vulnerable to model stealing~\citep{SSLextraction,StolenEncoder,ContSteal} than previous supervised models. 

Most of the current defenses against encoder stealing are \textit{reactive}, \ie they do not actively prevent the stealing but rather aim at detecting it by adding watermarks to the encoder~\citep{SSLguard, SSLextraction} or performing dataset inference to identify stolen copies~\citep{SSLdatasetinference}.
Since at the point of detection, the damage of stealing has already been inflicted,
%and it is unclear how ownership resolution of encoders can be settled in practice 
we argue that reactive defenses intervene too late and we advocate for \textit{active} defenses that prevent stealing while it is happening.
Yet, active defenses are challenging to implement because they do not only need to prevent the stealing but they also should preserve the utility of representations for legitimate users.
The only existing active attack against encoder stealing~\citep{StolenEncoder} falls short on this latter aspect since it significantly degrades the quality of representations for all users.


\franzi{B4B is a framework that consists of 3 building blocks:
1. Tracking embedding space coverage for user representations
2. The cost function that based on the coverage noises the user's representations
3. the transformations that fight off sybils
All of them can be instantiated with different functions.
We propose a concrete instantiation based on...}

\vspace{-0pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/schema/schema-active-defense.pdf} %width=\linewidth
    %\caption{\textbf{Overview of P2P Learning}. Every peer can act as a client (to compute updates) or server (to aggregate updates). \textcolor{blue}{Blue} represents semi-honest while \textcolor{red}{red} is the malicious setting.}
    \caption{
    \textbf{Overview of \name.} \encircle{1} Querying party sends an image to the API to obtain a representation. \encircle{2} For a single-account defense, we compute the query cost based on the number of buckets filled in by the querying user. The output representations are noised based on the computed cost to lower the fidelity of the extraction. \encircle{3} To prevent multi-account attacks, we apply a transformation, which is unique per user, to the original output representation. This prevents sybils from unifying representations from many accounts. \encircle{4} Querying party receives transformed and potentially noised representations.
    }
    \label{fig:b2b-overview}
\vspace{-0pt}
\end{figure}


To close the gap between required and existing defenses, we propose \textit{Bucks for Buckets (B4B)}, the first active defense against encoder stealing that does not harm utility for legitimate users.
B4B leverages the observation that the representations returned to adversaries who try to steal the encoder's functionality cover a significantly larger fraction of the full embedding space than representations of legitimate users who utilize the encoder to solve a particular downstream task.
Our defense tracks per-user embedding space coverage by employing local sensitive hashing that maps any representation returned to them into a set of \textit{hash buckets}.
B4B then adaptively adjusts the \textit{costs} for incoming user-queries according to the fraction of buckets already occupied by their representations.
We choose to employ representation utility as a cost function.\footnote{Note that our B4B allows to integrate multiple alternative cost functions, that rely on, for example, monetary costs, \ie increase the per-query-batch price with increasing coverage, or on costs in terms of an increasing amount of computations required by the users to obtain their representations, similar to a Proof-of-Work~\citep{powDefense}.}
More precisely, we design B4B such that it adds noise with a magnitude that increases with the number of buckets occupied by a given user to their representations before returning them. 
While the scale of noise added to legitimate users' representations does not harm their downstream performance due to their small embedding space coverage, the representations returned to an adversary become increasingly noisy---significantly degrading the performance of their stolen encoder.


To prevent adaptive attackers from circumventing our defense by creating multiple user-accounts (sybils) and distributing their queries over these accounts such that they minimize each account's utility drop, we equip B4B with per-user transformations that are applied to their returned representations.
Prior work has observed that certain types of transformations (\eg affine transformations, shuffling, padding) do not harm the performance of downstream tasks~\citep{SSLdatasetinference} and hence preserve the utility for legitimate users within B4B.
%As a result, B4B's per-user transforming do not harm utility for legitimate users.
In contrast, an adversary, cannot directly combine the representations obtained through different accounts anymore to train their stolen copy of the encoder.
Instead, they first have to remap all representations into the same embedding space, which we show requires a significant query and computation overhead and still reduces performance of the stolen encoder.\tf{These latter, we need to verify them in the experiments and potentially weaken the text.}
%\franzi{End on something like: "We empirically show that to learn good remappings, the adversary requires Xk queries (same queries from multiple accounts) which makes the effort not worth and the stealing impractical.}
We present the end-to-end design of B4B in \Cref{fig:b2b-overview}.

% We introduce an effective method to actively defend encoder stealing. 
% Our work addresses the lack of active defenses against stealing encoders that prevent attacks as they are happening without degrading the performance of legitimate users.
%As presented in \Cref{fig:b2b-overview}, we compute the query cost based on the occupied output space by a given user's representations. Our defense decreases the fidelity of representations when more output space is covered by single-user queries to disincentivize attackers from stealing the SSL encoders. Alternatively, the API providers could use other methods to either lower the quality of outputs or increase the cost of extraction, for example, by increasing the price per batch of queries or requiring users to complete a proof of work, disk space, or time.
%Our approach makes the querying for a single user more expensive when the number of queries increases and the growth in cost is higher with a greater spread of extracted representations. Then, if an attacker wants to create more accounts to lower the cost of stealing, the mapping of the representations to the same space is even more expensive, thus, preventing the extraction of encoders. 
% Then, if attackers would like to circumvent the single-user defense and avoid noisy answers, they can revert to Sybil attacks, where adversaries create many fake accounts and query an API from each of them instead of funneling all queries through a single user.
% % We suggest that it is possible 
% To prevent such attacks, we harden our defense by returning differently transformed representations to each user. 
% Examples of such transformations include affine transformations, a shuffle of elements in the representations, or a combination of such operations.
% The transformations do not harm the performance on downstream tasks~\citep{SSLdefense} but modify the representations for different accounts, such that an adversary would have to find the mappings between differently transformed representations.
% The mapping is even more expensive in terms of the number of required queries, thus, preventing the extraction of encoders. 
% %In contrast, since owners of APIs are the ones to apply the transformations, they can also easily reverse them to identify stolen copies.



% On a single-user level, the APIs providers should ensure that a given user operates within a single account to solve a given task. 
% Our analysis shows that single-domain tasks tend to have representations concentrated within a single subspace of the representation space instead of being spread through the whole space. 
% If a user's queries are dispersed and come from many downstream tasks, such a user is penalized to disincentive the stealing. 
% Since querying the API for multiple tasks as a single user is prohibitive, an attacker can try to create Sybil accounts. Our method creates distinct transformations of output representations per account such that it does not lower the quality of outputs for legitimate users but makes the cost of remapping between representations surge. This prevents an attacker from reunifying all the representations and training the stolen copy of the victim encoder.

% In Sybil attacks, adversaries create many fake accounts and query an API from each of them instead of funneling all queries through a single user.
% % We suggest that it is possible 
% To prevent such attacks, we can harden both of our defense methods by returning differently transformed representations to each user. 
% Examples of such transformations include affine transformations, a shuffle of elements in the representations, or a combination of such operations.
% The transformations do not harm the performance on downstream tasks~\citep{SSLdefense} but modify the representations for different accounts, such that an adversary would have to find the mappings between differently transformed representations.
% In contrast, since owners of APIs are the ones to apply the transformations, they can also easily reverse them to identify stolen copies.

In summary, we make the following contributions:
\begin{enumerate}
    \item We propose \name, the first active defense against stealing encoders that does not harm downstream performance for legitimate users. \name decreases the quality of representations returned to a given user according to their coverage of the embedding space. 
    \item We extend B4B to be resilient against sybil attacks.
    %To prevent Sybil attackers, who create many fake accounts, we output differently transformed representations to each user such that the remapping to a unified space between representations is prohibitively costly.
    Therefore, we rely on per-user transformations for the returned representations which makes combining representations from different accounts inefficient for encoder stealing.
    \item We show how to calibrate the cost function in B4B and provide an end-to-end evaluation of our defense to highlight its effectiveness in encoder stealing scenarios.
    %that shows how to calibrate the defense against a single-user attacker, how the transformations per account effectively prevent Sybil adversaries, and finally present an end-to-end experiment which shows how our defense performs in realistic scenarios.
\end{enumerate}
